FedCross: Towards Accurate Federated Learning via Multi-Model Cross-Aggregation

As a promising distributed machine learning paradigm, Federated Learning (FL) has attracted increasing attention to deal with data silo problems without compromising user privacy. By adopting the classic one-to-multi training scheme (i.e., FedAvg), where the cloud server dispatches one single global model to multiple involved clients, conventional FL methods can achieve collaborative model training without data sharing. However, since only one global model cannot always accommodate all the incompatible convergence directions of local models, existing FL approaches greatly suffer from inferior classification accuracy. To address this issue, we present an efficient FL framework named FedCross, which uses a novel multi-to-multi FL training scheme based on our proposed multi-model cross-aggregation approach. Unlike traditional FL methods, in each round of FL training, FedCross uses multiple middleware models to conduct weighted fusion individually. Since the middleware models used by FedCross can quickly converge into the same flat valley in terms of loss landscapes, the generated global model can achieve a well-generalization. Experimental results on various well-known datasets show that, compared with state-of-the-art FL methods, FedCross can significantly improve FL accuracy within both IID and non-IID scenarios without causing additional communication overhead.

==> response.tex <==
\clearpage
\setcounter{section}{0}

\newcounter{cntcmmt}




\newcommand{\Cmnt}[1]
{ \noindent {\bf Comment \stepcounter{cntcmmt}\arabic{cntcmmt}:}
{\it #1} \vspace{0.05in} }



\newcommand{\Rsp}[1]
{\noindent {\bf Response:} #1 \vspace{0.09in}}



\def\commref#1{Comment~\ref{#1}}

\section*{Responses to Reviewers' Comments}

%\textcolor[rgb]{1,0,0}{{\bf Note that 
%the original  log number of this manuscript is TC-2019-01-0001.R2}}.

We would like to thank the meta-reviewer and all the reviewers for their thorough and insightful comments. We have revised the manuscript to address various issues raised by the reviewers. 
This section presents our responses to all the reviewers' comments in a point-to-point fashion. 

%in terms of how we have addressed the issues in the revision


\subsection{Meta-Reviews}
\begin{tcolorbox}
[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{The reviewers agree that the paper is interesting but they want to see several major changes before the paper can be accepted to ICDE.\\
See point 12 of the individual reviews.
}
\end{tcolorbox}
\Rsp{We thank the meta-reviewer and reviewers for your helpful comments. In this revised draft, we have addressed all the comments (including Point 12 of individual reviews) and greatly improved the quality of our paper. Please refer to the details of our responses below.

}


\subsection{REVIEWER \#2}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{O1: Main contributions (in particular proofs) seem to be on areas not really within the scope of ICDE.
%, as is also evident from venues most of the references come from.
}
\end{tcolorbox}
\Rsp{
The main contribution of our paper is that it presents a novel multi-to-multi FL framework, named FedCross, to address the performance degradation problem 
caused by the non-IID data of clients.
To evaluate the effectiveness of our method, we present theoretical proofs to demonstrate the convergence of our FedCross approach.
Since FedCross aims to deal with heterogeneous data problems in federated learning, according to ``Call for Research Papers'' of ICDE (\textit{https://icde2024.github.io/CFP\_research.html}),
our work belongs to the areas of ``Distributed, Parallel, and P2P Data Management'', ``IoT Data Management'', and ``AI for Database Systems''.
Please note that in recent years, many works [R1-R3] focusing on FL appeared in ICDE.

\noindent\underline{\bf \small References}

\noindent\textit{
\footnotesize
[R1] FedKNOW: Federated Continual Learning with Signature Task Knowledge Integration at Edge. ICDE 2023: 341-354
}

\noindent\textit{
\footnotesize
[R2] Distribution-Regularized Federated Learning on Non-IID Data. ICDE 2023: 2113-2125.
}

\noindent\textit{
\footnotesize
\noindent[R3] Federated Learning on Non-IID Data Silos: An Experimental Study. ICDE 2022: 965-978.
}
}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{O2: The datasets are relatively small. In the papers describing the baselines (e.g., [32]), datasets are larger (and probably more realistic). It's very possible that this selection of datasets (without a good reason for the selection, as the larger ones are also available) favors the proposed approach.}
\end{tcolorbox}
\Rsp{We thank the reviewer for your helpful suggestions. In this revised draft, in order to demonstrate the scalability of our approach, we conducted a new set of experiments on larger datasets, ShakeSpeare and Sent140 datasets, which were used in [32]. Since ShakeSpeare and Sent140 are text datasets rather than image datasets, we cannot use CNN, ResNet, or VGG. 
For these two datasets, the same as [32], we used the LSTM model and conducted their build-in data distributions in our experiments.
Note that, in the previous version, we conducted the experiment on the FEMNIST dataset as the one used in [32].
%In our previous version, we also conducted experiments on an image dataset (i.e., FEMNIST) used in [32].
New experimental results on ShakeSpeare and Sent140 datasets have been reported in the last two rows of Table~\ref{tab:acc}, respectively.
We can observe that FedCross achieves the best inference accuracy compared with all the baselines for both large datasets.
}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{O3: Not all relevant hyperparameters for baselines described, e.g. \# rounds.}
\end{tcolorbox}
\Rsp{
Thanks very much for pointing out this. 
For all the baselines, we set the number of rounds to 2,000 when using CNN and ResNet-20 models, and set it to 1,000 when using the VGG-16 model. 
We have revised the first paragraph of Section~\ref{sec:exp_acc} to clarify this experimental setting.
}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{O4: Not clear how the datasets are distributed over the clients.}
\end{tcolorbox}
\Rsp{
Thanks for your insightful comments. To display the Dirichlet distribution in a more intuitive way, in this revision, we have added new figures, Figures~\ref{fig:data_dis}(a)-~\ref{fig:data_dis}(c) to 
show the data distributions of 10 
clients for the experiment on the CIFAR-10 dataset, which are randomly selected from all the 100 clients.  
In these subfigures, the samples on clients follow the 
% out of 100 clients, where the data of clients are divided from CIFAR-10 dataset, following 
the Dirichlet distributions with $\beta= 0.1$, $0.5$, and $1.0$, respectively.
We have included Figure~\ref{fig:data_dis} and its corresponding discussions in Section~\ref{sec:exp_setting}.
}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{O5: Not clear whether the baselines are reimplemented/interpreted or based on publicly available code.}
\end{tcolorbox}
\Rsp{
Thank you very much for your comments. 
We implemented/adapted all the baselines and our proposed approach under our own unified FL framework. For those baselines such as FedGen and CluSamp, we re-used the publicly available code from \cite{fedgencode} and \cite{clusampcode}, respectively. For the remaining baselines, since we could not find the available code, we re-implemented these baselines based on the descriptions in the papers \cite{li2020federated,karimireddy2020scaffold}.





%Since all the experiments are conducted on the same federated framework, we implemented all the baselines under our framework.
%Please note that the implementations of each baseline were reimplemented based on its publicly available code and relative paper.
}


\subsection{REVIEWER \#6}
\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{O1: The paper needs more clarification about why the multi-model framework works. From Table 1, even though in the IID setting, FedCross outperforms the other baselines. Basically, FedCross organizes the clients into pairs and conducts FedAvg within each pair in each round. There is no guarantee that the model will finally converge to the flat optimal as shown in Fig 1 (b). More justification is needed for the effectiveness of FedCross.}
\end{tcolorbox}
\Rsp{
Thank you very much for your insightful comments. In the last version, we conducted experiments to validate that the model trained by FedCross can converge to a  flatter optimal than the one achieved by FedAvg. Please refer to 
Figure~\ref{fig:val_landscape} of Section~\ref{sec:exp_val}
for more details. 
% The experimental results are shown in Figure~\ref{fig:val_landscape} of Section~\ref{sec:exp_val}.
Note that Figure~\ref{fig:val_landscape} illustrates the loss landscapes of global models trained by FedAvg and FedCross based on their corresponding datasets.
We can observe that the global models trained by FedAvg are located in sharper areas compared with the ones obtained by FedCross. 
This reveals that all the clients converge
toward flatter optimal solution areas, which is consistent with our observation in Figure~\ref{fig:motivation}.
In other words, from the perspective of loss landscapes, FedCross can train a more generalized global model than 
FedAvg. 
%
Note that even for an IID scenario, the global model trained by FedAvg can still fall into a relatively sharp area within some loss landscape.
% , though such a solution is flatter than the solutions obtained
% in non-IID scenarios. 
%Compared with 
%FedAvg,  
In this case, due to the effect of our proposed multiple-to-multiple training scheme, FedCross can easily guide the optimized model toward a  flatter area.
In summary, FedCross outperforms other FL methods for both IID and non-IID scenarios.
}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{O2: Scalability of FedCross. When the number of selected clients increases, the number of models also increases, which incurs large storage overhead.
}
\end{tcolorbox}
\Rsp{
Thanks for your useful comments. 
We have already conducted the experiment by varying the numbers of selected clients in Figure~\ref{fig:frac}.
To investigate the scalability of FedCross, we conducted a set of new experiments for different numbers of clients (i.e., $|C|=50$, $100$, $200$, $500$, and $1,000$) on the CIFAR-10 dataset, based on the ResNet-20 model within a non-IID scenario ($\beta=0.5$). For each case, we selected 10\% of the clients to participate in local training.
Specifically, Figure~\ref{fig:client_num} shows the learning curves of FedCross and five baselines with different settings of the total number of clients.
We can observe that FedCross can achieve the best inference accuracy for all the cases. 
Note that
in this experiment, since the total number of samples is fixed,
the larger the total number of clients, the smaller the amount
of data assigned to each client. As a result, we can find that
when the number of clients increases, all the investigated FL
methods need to use more training rounds for convergence.
% We can also see that with the increase of the total number of clients, all the methods will spend more training rounds for convergence.
% This is because the larger the total number of clients, the smaller the amount of data assigned to each client.
We have included Figure~\ref{fig:data_dis} and its discussions to Section~\ref{sec:exp_client_num}.
}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{O3: There are many FL studies working on the simulated FL setting by partitioning the image datasets, and such a setting is not attractive nowadays. I suggest the authors add some real federated datasets to make the experiments more solid.}
\end{tcolorbox}
\Rsp{
Thank you very much for your helpful comments. 
In this revision, in order to demonstrate the scalability of our approach, we conducted a new set of experiments on larger datasets, ShakeSpeare and Sent140 datasets, which were used in [32]. Since ShakeSpeare and Sent140 are text datasets rather than image datasets, we cannot use CNN, ResNet, or VGG.
For these two datasets,  we conducted the experiments based on  the LSTM model and used their build-in data distribution. 
% In the same way as [32], for these two datasets,  we used the LSTM model and conducted their build-in data distributions in our experiments.
% In our original draft, we also conducted experiments on an image dataset (i.e., FEMNIST) used in [32].
New experimental results on ShakeSpeare and Sent140 datasets have been reported on the last two rows of Table~\ref{tab:acc}, respectively.
We can observe that FedCross achieves the best inference accuracy compared with all the baselines for both large datasets.
}


%To demonstrate the effectiveness of our approach on larger datasets, in our revision version, we conducted extended experiments on ShakeSpeare and Sent140 datasets.  Please note that all the two datasets are still used in [32]. Sicne ShakeSpeare and Sent140 are text datasets rather than image datasets, we cannot use CNN, ResNet, or VGG. For the two datasets, same as [32], we used the LSTM model and conducted their build-in data distribution in our experiments. Please note that [32] conducted experiments on an image dataset (i.e., FEMNIST), which has already been used in our initial version. The experimental results are presented in the $30^{th}$ and $31^{th}$ rows of Table~\ref{tab:acc}. We can observe that FedCross achieves the best inference accuracy compared with all the baselines in both cases.


\subsection{REVIEWER \#8}
\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{O1: It would be great to clarify the functional differences between the approach and existing works, e.g. a table to compare their functionalities or aspects.}
\end{tcolorbox}
\Rsp{
Thanks for your useful suggestions. In this revision, we have clarified the functional differences between the FedCross and existing works by adding  Table~\ref{tab:baseline} and its discussions in Section~\ref{sec:exp_setting}.
Table~\ref{tab:baseline} presents the category and communication overhead for FedCross and all the five baselines.
Since FedCross, as a novel FL method, cannot be classified into any of the existing three categories, we classify it as a new category, i.e., multi-model
guided method.
}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{O2: Some detailed proofs can be summarized and moved to the appendix to make the reading flow easier.}
\end{tcolorbox}
\Rsp{
We thank the reviewer for your helpful suggestions. We would like to put detailed proofs to the appendix for clearer presentation. However, the submission guideline of the ICDE conference does not allow the appendix (``{\it No appendix is allowed}'' from \textit{\url{https://icde2024.github.io/CFP_research.html}}). Therefore, we have to present all the proofs within the main body of the paper. 
As suggested by the reviewer, in this revised draft, we have simplified/summarized the proofs to make the reading flow easier, and deleted some unnecessary intermediate derivation steps.
}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\Cmnt{O3: It is mentioned that ``Although all the above methods can improve FL performance from different perspectives, since they are based on the coarse-grained one-to-multi FL training scheme, their learning capabilities are severely limited.'' It would be great to summarize of elaborate more on the concrete limitations of existing works. Some examples might help.}
\end{tcolorbox}
\Rsp{
Thank you for your helpful suggestions.
Due to the usage of the same global model for local training,
existing FL methods greatly suffer from
the problem of getting stuck in sharp ravines during the
exploration of loss landscapes. As an alternative,  FedCross
 adopts multiple intermediate models for local training. In this case,  intermediate models can quickly escape
from  sharp areas based on our proposed cross-aggregation
mechanism.
% existing methods are easily stuck in a sharpness area. Unfortunately, these methods do not have a strategy to guide the model to come out of the sharpness areas.
% In contrast, our FedCross approach adopts multiple intermediate models for local training. As a result, even if some models fall into a sharpness area, they can still be guided to come out of such a sharpness area through the cross-aggregation mechanism.
We added the discussion above to the $4^{th}$ paragraph of Section~\ref{sec:relwork}.
}


